Latent Topology Induction for Understanding Contextualized Representations

In this work, we study the representation space of contextualized embeddings and gain insight into the hidden topology of large language models. We show there exists a network of latent states that summarize linguistic properties of contextualized representations. Instead of seeking alignments to existing well-defined annotations, we infer this latent network in a fully unsupervised way using a structured variational autoencoder. The induced states not only serve as anchors that mark the topology (neighbors and connectivity) of the representation manifold but also reveal the internal mechanism of encoding sentences. With the induced network, we: (1). decompose the representation space into a spectrum of latent states which encode fine-grained word meanings with lexical, morphological, syntactic and semantic information; (2). show state-state transitions encode rich phrase constructions and serve as the backbones of the latent space. Putting the two together, we show that sentences are represented as a traversal over the latent network where state-state transition chains encode syntactic templates and state-word emissions fill in the content. We demonstrate these insights with extensive experiments and visualizations.

==> 050discovery.tex <==
\subsection{State-Word Emissions}

\paragraph{Decomposing the Meaning of Learned States}
Classes not mutually exclusive. 
(1). from random tag to random embedding (2). from random embedding to Bert embedding (3). Bert Zero v.s. Bert Last. DEP aligns with the supervised probing results but bypasses its dilemma (4). Later on not aligned states and effect of contextualization. (5). Again, emphasize that the granularity of the meaning is much finer than POS and NER.


\paragraph{Case Study.The Mechanism of Contextualization} 

TODO: Table 1. subwords before and after contextualization 

TODO: Table 2. morphological clusters

TODO: Table 3. Failure modes

(1). encoding of subwords: before contextualization, subwords are just forms without meaning, contextualization gives them meaning, and these meanings are induced from their context, which is precisely the basic assumption of distributional semantics. 

(2). encoding of stopwords. TBC

(3). evidences of things not understood after contextualization. 

\paragraph{States not Alignment with Predefined Knowledge} Human Annotation on what they encode; Give top 10 state example


\subsection{State-State Transitions}


\paragraph{State-state Visualization}
encoding of stopwords. Again the mechanism of contextualization. 


\subsection{The Mechanism of Sentence Encoding within the Representation Space}

==> 099_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The abstract and introduction are basically one-to-one summarizaion of the model and experiments sections}
  \item Did you describe the limitations of your work?
    \answerYes{See the conclusion section}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our methods is more about theoretical analysis of large language models}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{Our hypothesis is evidenced by experiments, not proofs}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We do not have enough time to organize the code, but we will update upon acceptance}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See experiment section}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{Our method is more about analytics}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{we do not know what the license is}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{but 20News is a widely used standard dataset}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{But during our inpection, we did not find any}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{They are paid with the average local hour rate.}
\end{enumerate}


\end{enumerate}

==> fig_state_freq.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figs/state_freq}
  \caption{Decomposing representation space into a spectrum of latent states. Each bar represents a latent state with height equals to log frequency. Aligned (or not aligned) = states aligned (or not aligned, see Table~\ref{tab:overall} and~\ref{tab:not_aligned}) with existing linguistic annotation. States from \textsc{BertLast} are more contextualized ($\approx$ more blue and green bars) than \textsc{BertZero}. 
  }
  \label{fig:state_freq}
\end{figure*}


==> tab_align_not_align.tex <==
\begin{table*}[t!]
  \small
  \caption{\label{tab:overall}Decomposing representation space by aligning to existing linguistic annotation. \#s = number of states, \%c = percentage of covered word occurrence. Generally, \colorbox[HTML]{FFC897}{POS} and \colorbox[HTML]{FFC897}{ENT} can be inferred from the word directly while
   \colorbox[HTML]{DAE8FC}{DEP}, \colorbox[HTML]{DAE8FC}{CCG} and  \colorbox[HTML]{DAE8FC}{BCN} require more context.  
  We observe the most aligned states inferred from \textsc{BertLast} (contextualized) 
%   than \textsc{BertZero} (non-contextualized), especially 
  for tags requiring contextualization. 
  }
  \begin{center}
  \scriptsize
  \begin{tabular}{@{}lcccccccccccccccc@{}} 
  \toprule
  &  \multicolumn{2}{c}{\colorbox[HTML]{FFC897}{POS}} 
  & \multicolumn{2}{c}{\colorbox[HTML]{DAE8FC}{DEP}} & \multicolumn{2}{c}{\colorbox[HTML]{DAE8FC}{CCG}} & \multicolumn{2}{c}{\colorbox[HTML]{DAE8FC}{BCN}} &  \multicolumn{2}{c}{Not Aligned}  \\ 
  & \#s & \%c & \#s & \%c & \#s & \%c  & \#s & \%c & \#s & \%c \#s & \%c \#s & \%c \#s & \%c \\
  \midrule
  \textsc{Positional} & 3 & 0.4  & 3 & 0.4 & 1& 0.01 &1 & 0.01 & 1997 & 99.5 & - & - & - & - & - & - \\
  \textsc{RandEmb} & 392 & 53.0 & 366 & 52.3  & 241 & 45.2 & 334 & 49.1 & 1159 & 43.4 & - & - & - & - & - & - \\ 
  \textsc{BertZero} & 673 & 65.3 & 468 & 53.8 & 450 & 51.8 & 275 & 48.8 & 1253 & 27.6 & - & - & - & - & - & - \\ 
  \textsc{BertLast} & 804 & 53.2 & 740 & 42.6 & 583 & 44.0 & 628 & 44.5 & 1069 & 40.5 & - & - & - & - & - & - \\ 
  \bottomrule
  \end{tabular}
  \end{center}
\end{table*}




==> tab_not_know.tex <==

\begin{table*}[t!]
  \small
  \caption{\label{tab:not_know} \small Examples of concept \textit{not understood} by contextualization. 
  }
  \begin{center}
  \begin{tabular}{@{}p{2.5cm}p{5.3cm}p{5.3cm}@{}} 
  \toprule
  & Before Contextualization (\textsc{BertZero}) & After Contextualization (\textsc{BertLast})\\ 
  \midrule
  Good v.s. bad &  & \\ 
  Hard v.s. easy &  & \\ 
  True v.s. false &  & \\ 
  Increase v.s. reduce &  & \\ 
  \bottomrule
  \end{tabular}
  \end{center}
\end{table*}
